PhysDreamer: Physics-Based Interaction with 3D Objects via Video Generation

Realistic object interactions are crucial for creating immersive virtual experiences, yet synthesizing realistic 3D object dynamics in response to novel interactions remains a significant challenge. Unlike unconditional or text-conditioned dynamics generation, action-conditioned dynamics requires perceiving the physical material properties of objects and grounding the 3D motion prediction on these properties, such as object stiffness. However, estimating physical material properties is an open problem due to the lack of material ground-truth data, as measuring these properties for real objects is highly difficult. We present PhysDreamer, a physics-based approach that endows static 3D objects with interactive dynamics by leveraging the object dynamics priors learned by video generation models. By distilling these priors, PhysDreamer enables the synthesis of realistic object responses to novel interactions, such as external forces or agent manipulations. We demonstrate our approach on diverse examples of elastic objects and evaluate the realism of the synthesized interactions through a user study. PhysDreamer takes a step towards more engaging and realistic virtual experiences by enabling static 3D objects to dynamically respond to interactive stimuli in a physically plausible manner. See our project page at https://physdreamer.github.io/.

==> sections/01_introduction.tex <==
\section{Introduction}
\label{sec:intro}

Object dynamics play a pivotal role in our perception of the visual world. 
When envisioning a rose, 
we not only picture its appearance, 
but also vividly see how it gently sways in reaction to a breeze or a delicate touch.
Such {\it interactive} dynamics is essential for a complete and lifelike representation of objects in our minds.
Recent advances in 3D vision have enabled the capture and creation of high-quality static 3D assets, allowing for realistic rendering from any viewpoint~\cite{mildenhall2020nerf,gaussiansplat2023}. 
However, accurately modeling object dynamics under interactions remains a significant challenge.

In this work, we focus on synthesizing 3D object dynamics under physical interactions. 
Our goal is to transform a given \emph{static} 3D object and make it \emph{interactive}, enabling the simulation of its dynamic responses to novel interactions from an agent or the environment, such as natural forces like wind or human interactions like poking and dragging.
Such interactivity is important for creating truly lifelike virtual experiences and synthesizing agent interactions with objects. 


\input{fig_txt/fig_teaser}

The key challenge in simulating realistic interactive 3D dynamics lies in accurately estimating an object's physical material properties. 
These properties are crucial for motion realism but are not readily available from a static 3D model alone. 
Real-life objects often exhibit complex, spatially-varying material properties, such as a rose with soft petals and a sturdy stem, or a plush toy with a fluffy exterior and a dense filling. 
Estimating such material properties solely from a static 3D representation is an open problem due to the lack of ground-truth data: Accurately measuring physical material properties is highly costly, and manually annotating them is even more difficult.


To address this problem, we propose \textbf{\model}, an approach to estimating physical material properties for a static 3D object by distilling the dynamics priors from a video generation model. 
The key idea is that, since video generation models learn a prior over object dynamics from large amount of videos, they could animate daily objects in their common motion which is governed by their physical material properties. In other words, a well-trained video generation model may implicitly bridge object appearance to object dynamics. Therefore, we explore distilling the object dynamics priors from a video generation model to estimate the governing physical material properties.

In particular, our approach, \model, synthesizes plausible videos of a 3D object in motion by a video generation model, and then optimizes a physical material field such that rendered videos of a simulation course match the generated videos. 
In particular, we represent the 3D object by 3D Gaussians~\cite{gaussiansplat2023} that supports differentiable rendering, we model the physical material field of the object by a neural field~\cite{xie2022neural}, and we simulate the 3D dynamics by the differentiable Material Point Method (MPM)~\cite{apicjiang2015, physgaussianxie2023, mlsmpmhu2018}.
The differentiable simulation and rendering allow us to optimize the physical material field and initial velocity field directly by matching pixel space observations. 
Once optimized, the resulting physical material properties enable realistic simulation of the object's 3D dynamics under novel interactions.

In this work, we focus on elastic dynamics and showcase \model through eight diverse real examples, including flowers, an alocasia plant, a telephone cord, and a beanie hat. 
To evaluate the realism of our synthesized motion, we conduct a user study comparing our results to two recent state-of-the-art methods and we show that our synthesized 3D dynamics are highly preferred over the recent methods. In terms of motion realism, our synthesized results are sometimes even favored by users over real captured videos. 




% Version-1. 
% Motion is crucial in our perception of the visual world.  When thinking about a rose, one readily pictures its color, texture from multiple angles. This visual imagery extends beyond static appearances, allowing one to vividly imagine its oscillatory movements in response to wind or touch. Without this gentile yet lifelike motion, our visual imagination remains incomplete. Recent advances in 3D vision enables high-quality capture, and creation of static 3D assets,  enabling realistic rendering from any viewpoint. However, accurately modeling the dynamics of objects, particularly in synthesizing the realistic motions of 3D objects during interactions, such as a rose's natural sway in response to external forces, remains a significant challenge.

% Data-driven approaches have significantly advanced the modeling of scene dynamics in 2D image space,  featuring video generative models\cite{imagenvideo2022, makeavideo2022, alignyourlatents2023, svdblattmann2023, emuvideo2023, animatediff2023, lumiere2024, sora2024}. These models excel at generating short videos with consistent and realistic motions.  However, the progress in data-driven modeling of 3D object dynamics has been limited, likely due to data scarcity and unclear representations.   A few studies have attempted to extend video generative models to synthesize 3D motions using techniques such as score distillation sampling. Yet, these methods are currently limited to producing fixed-length 3D videos, incapable of synthesizing interactive motions.   Synthesizing realistic motion for objects under novel physical interactions continues to be an unresolved issue.

% In this paper, we address the problem of synthesizing realistic 3D object motions under physical interactions. Our goal is to make a given 3D object interactable, allowing us to synthesize its dynamic responses to any novel forces, such as poking or pulling. We use 3D Gaussians~\cite{} as the underlying representation and material point methods~\cite{} for simulation.  A key challenge lies in accurately estimating the object's physical material parameters, which are crucial for realistic motion synthesis but often infeasible to compute or measure directly from a static 3D model. \TYZ{Split to a new paragraph here?} To address this issue, we propose a novel approach that uses video diffusion models to extract physical material parameters. We begin by rendering the 3D object from a specific viewpoint and use the rendered image as the initial frame for the video diffusion model. The model then generates short video clips depicting the object in motion. Next, through differentiable simulation and rendering, we optimize a set of spatially-varying physical material parameters and initial velocity to align with the video clip. Afterward, the optimized physical material parameters enable realistic simulation of the object's dynamics under any new interaction, bridging the gap between static 3D models and their dynamic real-world counterparts for enhanced realism and interactivity.

% In this paper, we narrow our focus to elastic objects.  We demonstrate our approach on eight examples, including flowers, an alocasia plant, a telephone cord, and a beanie hat. Tarting with 3D Gaussian representations, we synthesize realistic material parameters for these objects. This enables us to simulate their motions under novel interactions. To evaluate the realism of our synthesized motion, we conduct a user study comparing our motions against three counterparts: motions simulated with random material parameters, real captured videos, and motions generated by the baseline method DreamGaussian4D \cite{dreamgaussian4d2023}. \TYZ{Do I need to mention that Dreamgaussian4D cannot do interactivity?} We believe our work has the potential to inspire broad applications in digital content creation, particularly for the development of interactive assets.

==> sections/03_background.tex <==
\section{Background}
\label{sec:background}

In our approach, we employ 3D Gaussians~\cite{gaussiansplat2023} to represent objects. This representation uses a set of anisotropic 3D Gaussian kernels to represent a 3D scene. 
3D Gaussians were introduced as an efficient method for 3D reconstruction and novel view synthesis from posed images, but its Lagrangian nature also enables the direct adaptation of particle-based physics simulators. 
Following PhysGaussian~\cite{physgaussianxie2023}, we use the Material Point Method (MPM) to simulate object dynamics directly on these Gaussian particles. 
Since 3D Gaussians mainly lie on object surfaces, an optional internal filling process can be applied for improved simulation realism\cite{physgaussianxie2023}.  
Here, we provide a brief introduction on the underlying physical model and how to integrate MPM into 3D Gaussians. 
For a more comprehensive introduction of MPM, we refer the reader to \cite{materialjiang2016, apicjiang2015, mlsmpmhu2018, physgaussianxie2023}. 

\subsection{Continuum mechanics and elastic materials}

Continuum mechanics models material deformation using a map $\phi$ that transforms points from the undeformed material space $\mathbf{X}$ to the deformed world space $\mathbf{x} = \phi(\mathbf{X}, t)$. 
The Jacobian of the map, $\boldsymbol{F} = \nabla_{\mathbf{X}} \phi(\mathbf{X}, t)$, known as the deformation gradient, measures local rotation and strain.
This tensor is crucial in formulating stress-strain relationship. 
For example, the Cauchy stress in a hyper-elastic material is computed by: $ \bsigma = \frac{1}{\mathrm{det}(\bF)} \frac{\partial \psi}{\partial \bF} \bF^T$. 
Here, $\psi(\mathbf{F})$ represents the strain energy density function, quantifying the extent of non-rigid deformations.
This function is typically designed by experts, to follow principles like material symmetry and rotational invariance while aligning with empirical data. 
In this work, we use fixed corotated hyperelastic model, whose energy density function can be expressed as: 
\begin{equation}
    \label{eq:fixed-corotated}
\psi(\mathbf{F}) =  \mu \left( \sum_{i=1}^{d} (\sigma_i - 1)^2 \right) + \frac{\lambda}{2}(\mathrm{det}(\bF) - 1)^2,
\end{equation}
where $\sigma_i$ denotes a singular value of the deformation gradient. $\mu$ and $\lambda$ are related to Young's modulus $E$ and Poisson's ratio $\nu$ via: 
\begin{equation}
\label{eq:young_poisson}
    \mu = \frac{E}{2(1+\nu)}, \quad \lambda = \frac{E\nu}{(1+\nu)(1-2\nu)}. 
\end{equation}
The dynamics of an elastic object are governed by the following equations: 
\begin{equation}
    \begin{aligned}
        \rho \frac{D \bv }{D t} = \nabla \cdot \bsigma + \mathbf{f},  \quad
        \frac{D\rho}{Dt} + \rho \nabla \cdot \bv = 0,  \\
    \end{aligned}
\end{equation}
where $\rho$ denotes density, $\bv(\bx, t)$ denotes the velocity field in world space, and $\mathbf{f}$ denotes an external force. 


\subsection{Material point method}

We use the Moving Least Squares Material Point Method (MLS-MPM)~\cite{mlsmpmhu2018} to solve the above governing equation. 
MPM is a hybrid Eulerian-Langrangian method widely adopted for simulating dynamics for a wide range of materials, such as solid, fluid, sand, and cloth \cite{materialram2015, druckerklar2016, materialstomakhin2013, jiang2017anisotropic}.
MPM offers several advantages, such as easy GPU parallelization~\cite{hu2019taichi}, handling of topology changes, and the availability of well-documented open-source implementations~\cite{taichihu2019, warp2022, nclawma2023, physgaussianxie2023}.

Following PhysGaussian~\cite{physgaussianxie2023}, we view the Gaussian particles as the spatial discretization of the object to be simulated, and directly run MPM on these Gaussian particles.
Each particle $p$ represents a small volume of the object, and it carries a set of properties including volume $V_p$, mass $m_p$, position $\bx_p^t$, velocity $\bv_p^t$, deformation gradient $\bF_p^t$, and local velocity field gradient $\boldsymbol{C}_p^t$ at time step $t$. 

MPM operates in a particle-to-grid (P2G) and grid-to-particle (G2P) transfer loop. 
In the P2G stage, we transfer the momentum from particle to grid by: 
\begin{equation}
    m_i^t \bv_i^{t} = \sum_p N(\bx_i - \bx_p^t) [m_p \bv_p^t + (m_p\bC_p^t - \frac{4}{(\Delta x)^2} \Delta t V_p  \frac{\partial \psi}{\partial \bF} {\bF_p^t}^T )(\bx_i - \bx_p^t) ] + \boldsymbol{f}_i^t, 
\end{equation}
where the mass of the grid node $i$ is $m_i^t = \sum_p N(\bx_i - \bx_p^t) m_p$, $N(\bx_i - \bx_p^t)$ denotes the B-spline kernel, $\Delta x$ denotes the spatial grid resolution, $\Delta t$ denotes the simulation step size, and $\bv_i^{t}$ denotes the updated velocity on the grid. We then transfer the updated velocity back to the particles and update their positions as:
\begin{equation}
    \bv_p^{t+1} = \sum_i N(\bx_i - \bx_p^t) \bv_i^{t}, \quad \bx_p^{t+1} = \bx_p^{t} + \Delta t \bv_p^{t+1}. 
\end{equation}
Meanwhile, the local velocity gradient and deformation gradient is updated as: 
\begin{equation}
   \bC_p^{t+1} = \frac{4}{(\Delta x)^2} \sum_i N(\bx_i - \bx_p^t) \bv_i^{t} (\bx_i - \bx_p^t)^T,  \quad \bF_p^{t+1} = (\boldsymbol{I} + \Delta t \bC_p^{t+1}) \bF_{p}^{t}. 
\end{equation}


==> sections/04_method.tex <==
\section{Approach}
\label{sec:method}

\input{fig_txt/fig_young_example}

\subsection{Problem formulation}

Given a 3D object represented by 3D Gaussians $\{\mathcal{G}_p\}_{p=1}^P$, $\mathcal{G}_p = \{\bx_p, \alpha_p, \bm{\Sigma}_p, \bm{c}_p \}$ (where $\bx_p$ denotes the position, $\alpha_p$ denotes the opacity, $\bm{\Sigma}_p$ denotes the covariance matrix, and $\bm{c}_p$ denotes the color of the particle), our goal is to obtain physical material properties for each Gaussian particle $\mathcal{G}_p$, which enable realistic motion simulation under physical interactions. These properties include mass ($m_p$), Young's modulus ($E_p$), and Poisson's ratio ($\nu_p$).

Among these physical properties, Young's modulus $E_p$ plays a particularly important role in determining the object's motion under applied forces.
Intuitively, Young's modulus (Eq.~\ref{eq:young_poisson}) measures the material stiffness. 
A higher Young's modulus results in less deformation and more rigid and higher-frequency motion, while a lower value leads to more flexible and elastic behavior. We show an illustration in Fig.~\ref{fig:young}, which illustrates the simulated motion of a flower under the same applied forces but with different Young's modulus. 

Mass $m_p$ can be computed as the product of a constant density ($\rho$) and particle volume $V_p$. 
The particle volume can be estimated~\cite{physgaussianxie2023} by dividing a background cell's volume by the number of particles that cell contains. 
As for the Poisson's ratio $\nu_p$, we found that it has negligible impact on object motion in our preliminary experiments, and so we assume a homogeneous constant Poisson's ratio $\nu_p=\nu=0.3$. Therefore, our primary focus is on estimating the spatially varying Young's modulus for the 3D object.


\subsection{Overview}

Our key idea is to leverage a video generation model to synthesize plausible motions for a 3D object, and optimize the material properties to match this synthetic motion.
We begin by rendering a static image ($I_0$) using the 3D Gaussians under a specified viewpoint. We then leverage an image-to-video model (Stable Video Diffusion \cite{svdblattmann2023}) to generate a short video clip  $\{I_0, I_1, \ldots, I_T\}$ depicting the object's realistic motion. This generated video serves as our reference video. 
We then utilize differentiable simulation and differentiable rendering to optimize the physical scene properties (i.e., spatially varying Young's modulus) and an initial velocity field to match the object motion observed in the video. We specifically use rendered images rather than Gaussians' training images for the video generation, because we might not have access to training images((e.g., when 3D Gaussians are generated from text-to-3D models).). Also, rendered images preserve artifacts in 3D Gaussians, potentially simplifying later optimization process.
An overview of our method is shown in Fig.~\ref{fig:method_main}. 

\input{fig_txt/fig_overview}

\subsection{Estimating physical properties}
We adopt Moving Least Squares Material Point Method (MLS-MPM)\cite{mlsmpmhu2018, physgaussianxie2023} as our physics-based simulator, and employ the fixed corotated hyper-elastic material model for the 3D objects. The simulation process for a single substep is formalized as: 
\begin{equation}
    \bx^{t+1}, \bv^{t+1}, \bF^{t+1}, \bC^{t+1} = \mathcal{S}(\bx^{t}, \bv^{t}, \bF^{t}, \bC^{t}, \bm{\theta}, \Delta t),
\end{equation}
where $\bx^{t} = [\bx^t_1, \cdots, \bx_P^t]$ denotes the positions of all particles at time $t$, and similarly $\bv^{t} = [\bv^t_1, \cdots, \bv_P^t]$ denotes the velocities of all particles at time $t$. $\bF^{t}$ and $\bC^{t}$ denote the deformation gradient and the gradient of local velocity field for all particles, respectively. Both $\bF^{t}$ and $\bC^{t}$ are tracked for simulation purposes, not for rendering. $\bm{\theta}$ denotes the collection of the physical properties of all particles: mass $\bm{m} = [m_1, \cdots, m_P]$, Young's modulus $\bm{E} =[E_1, \cdots, E_P]$,  Poisson's ratio $\bm{\nu}=[\nu_1, \cdots, \nu_P]$, and volume $\bm{V}=[V_1, \cdots, V_P]$. $\Delta t$ is the simulation step size. 

We use a substep size $\Delta t \sim 1 \times 10^{-4}$ for most of our experiments. To simulate the dynamics between adjacent video frames, we iterate over hundreds of substeps since the time interval between video frames are typically tens of milliseconds.  For simplicity, we abuse notation to express a simulation step with $N$ substeps as:
\begin{equation}
    \begin{aligned}
    \bx^{t+1}, \bv^{t+1}, \bF^{t+1}, \bC^{t+1} = \mathcal{S}(\bx^{t}, \bv^{t}, \bF^{t}, \bC^{t}, \bm{\theta}, \Delta t, N)  \\
    \end{aligned}
\end{equation}
where the timestamp $t+1$ is ahead of timestamp $t$ by $N \Delta t$. 
After simulation, we render the Gaussians at each frame:
\begin{equation}
    \hat{I}^{t} = \mathcal{F}_{\mathrm{render}} (\bx^{t}, \bm{\alpha}, \bm{R}^{t}, \Sigma, \bm{c}),
\end{equation}
where $\mathcal{F}_{\mathrm{render}}$ denotes the differentiable rendering function, and $\bm{R}^{t}$ denotes the rotation matrices of all particles obtained from the simulation step.  

Using the generated video as reference, we optimize the spatially-varying Young's modulus $\bm{E}$ and an initial velocity field $\bv^0$ by a per-frame loss function:
\begin{equation}
\label{eq:rendering_loss}
L^t = \lambda L_{\mathrm{1}} (\hat{I}^t, I^t) + (1 - \lambda) L_{\mathrm{D-SSIM}} ( \hat{I}^t, I^t),
\end{equation}
where we set $\lambda=0.1$ in our experiments.

Rather than optimizing the material parameters and initial velocities jointly, we split the optimization into two stages for better stability and faster convergence. 
In particular, in the first stage, we randomly initialize the Young's modulus for each Gaussian particle and freeze it. 
We optimize the initial velocity field using only the first three frames of the reference video.  
In the second stage, we freeze the initial velocity and optimize the spatially varying Young's modulus field. 
During the second stage, the gradient signal only flows to the previous frame to prevent gradient explosion/vanishing.



\subsection{Accelerate simulation with subsampling}

High-fidelity rendering with 3D Gaussian Splatting typically requires millions of particles to represent a scene. Running simulations on all the particles poses a significant computational burden. To improve efficiency, we introduce a subsampling procedure for simulation, as illustrated in Figure~\ref{fig:subsample}.

Specifically, we apply $K$-means clustering to create a smaller set of driving particles $\{\mathcal{Q}_q\}_{q=1}^Q$ at $t=0$, where each driving particle is represented by $\mathcal{Q}^0_q = \{\bx^0_q, \bv^0_q, \bF^0_q, \bC^0_q, E_q, m_q, \nu_q, V_q\}$. 
The initial position of a driving particle $\bx_q^0$ is computed as the mean of the position $\bx_p$ of all cluster members. 
The number of the driving particles is much smaller than the number of 3D Gaussian particles, $Q \ll P$. 
We run simulations only on the driving particles. 
During rendering, we compute the position and rotation for each 3D Gaussian particle $\mathcal{G}_p$ by interpolating the driving particles. 
In particular, for each 3D Gaussian particle, we find its eight nearest driving particles at $t=0$, and we fit a rigid body transformation $\bm{T}$ between these eight driving particles at $t=0$ and at the current timestamp. This transformation $\bm{T}$ is applied to the initial position and rotation of the particle $\mathcal{G}_p$ to obtain its current position and rotation.

\input{fig_txt/fig_subsample}

\subsection{Velocity and material fields} 

Even with subsampling, the degree of freedom in the spatially-varying material is still high. In a typical scene, we have over ten thousand of driving particles, making the material estimation a highly ill-posed problem, where infinitely many solutions can lead to the same observation.

To address this problem, we induce a spatial smoothness prior by representing the initial velocity and Young's modulus as implicit neural fields, $E_q=f_\text{material}(\bx_q)$ and $\bv^0_q=f_\text{velocity}(\bx_q)$, rather than directly optimizing discrete values for all driving particles. 
In particular, we parameterize each field as tri-planes~\cite{peng2020convolutional,chan2022efficient} followed by a three-layer MLP. 
We adopt a total variation regularization for all spatial planes to further encourage smoothness in the optimized fields. Using $\bu$ to denote one of the 2D spatial planes, we write the total variation regularization term as: 
\begin{equation}
    \label{eq:tv_regularization}
    l_{\text{tv}} = \sum_{i,j} (u_{i+1, j} - u_{i,j})^2 + (u_{i, j+1} - u_{i,j})^2. 
\end{equation}

==> sections/04_method_new.tex <==
\section{Approach}
\label{sec:method}

\input{fig_txt/fig_young_example}

\subsection{Problem formulation}

Given a static 3D object represented by 3D Gaussians $\{\mathcal{G}_p\}_{p=1}^P$, $\mathcal{G}_p = \{\bx_p, \alpha_p, \bm{\Sigma}_p, \bm{c}_p \}$ (where $\bx_p$ denotes the position, $\alpha_p$ denotes the opacity, $\bm{\Sigma}_p$ denotes the covariance matrix, and $\bm{c}_p$ denotes the color of the particle), our goal is to estimate physical material property fields for the object to enable realistic interactive motion synthesis. These properties include mass $m$, Young's modulus $E$, and Poisson's ratio $\nu$.
Among these physical properties, Young's modulus $E$ plays a particularly important role in determining the object's motion under applied forces.
Intuitively, Young's modulus (Eq.~\ref{eq:young_poisson}) measures the material stiffness. 
A higher Young's modulus results in less deformation and more rigid and higher-frequency motion, while a lower value leads to more flexible and elastic behavior. We show an illustration in Fig~\ref{fig:young}, which illustrates the simulated motion of a flower under the same applied forces but with different Young's modulus. 

Therefore, our problem formulation focuses on estimating the spatially varying Young's modulus field $E(\bx)$ for the 3D object. In particular, we model $E(\bx)$ by an implicit neural field~\cite{xie2022neural} parameterized by triplanes~\cite{peng2020convolutional,chan2022efficient} followed by a three-layer MLP.
To allow particle simulation, we query a particle's property by $E_p=E(\bx_p)$.

As for other physical properties, the mass for a particle $m_p$ can be pre-computed as the product of a constant density ($\rho$) and particle volume $V_p$. 
The particle volume can be estimated~\cite{physgaussianxie2023} by dividing a background cell's volume by the number of particles that cell contains. 
As for the Poisson's ratio $\nu_p$, we found that it has negligible impact on object motion in our preliminary experiments, and so we assume a homogeneous constant Poisson's ratio $\nu_p=\nu=0.3$.


\subsection{Overview}

Our key idea is to generate a plausible video of the object in motion, and then optimize the material field $E(\bx)$ to match this synthetic motion.
We begin by rendering a static image ($I_0$) for the 3D scene $\{\mathcal{G}_p\}$ from a certain viewpoint. We then leverage an image-to-video model (Stable Video Diffusion \cite{svdblattmann2023}) to generate a short video clip $\{I_0, I_1, \ldots, I_T\}$ depicting the object's realistic motion. This generated video serves as our reference video. We then optimize the material field $E(\bx)$ and an initial velocity field $\bv_0(\bx)$ through differentiable simulation and differentiable rendering, such that a rendered video of the simulation matches (from the same viewpoint as $I_0$) the reference video.
An overview of our method is shown in Fig.~\ref{fig:method_main}.

\input{fig_txt/fig_overview}

\subsection{Estimating physical properties}
We adopt Moving Least Squares Material Point Method (MLS-MPM)\cite{mlsmpmhu2018, physgaussianxie2023} as our physics simulator, and employ the Fixed Corotated hyper-elastic material model for the 3D objects. The simulation process for a single substep is formalized as: 
\begin{equation}
    \bx^{t+1}, \bv^{t+1}, \bF^{t+1}, \bC^{t+1} = \mathcal{S}(\bx^{t}, \bv^{t}, \bF^{t}, \bC^{t}, \bm{\theta}, \Delta t),
\end{equation}
where $\bx^{t} = [\bx^t_1, \cdots, \bx_P^t]$ denotes the positions of all particles at time $t$, and similarly $\bv^{t} = [\bv^t_1, \cdots, \bv_P^t]$ denotes the velocities of all particles at time $t$. $\bF^{t}$ and $\bC^{t}$ denote the deformation gradient and the gradient of local velocity fields for all particles, respectively. Both $\bF^{t}$ and $\bC^{t}$ are tracked for simulation purposes, not for rendering. $\bm{\theta}$ denotes the collection of the physical properties of all particles: mass $\bm{m} = [m_1, \cdots, m_P]$, Young's modulus $\bm{E} =[E_1, \cdots, E_P]$,  Poisson's ratio $\bm{\nu}=[\nu_1, \cdots, \nu_P]$, and volume $\bm{V}=[V_1, \cdots, V_P]$. $\Delta t$ is the simulation step size. 

We use a sub-step size $\Delta t \sim 1 \times 10^{-4}$ for most of our experiments. To simulate the dynamics between adjacent video frames, we iterate over hundreds of sub-steps since the time interval between video frames are typically tens of milliseconds.  For simplicity, we abuse notation to express a simulation step with $N$ sub-steps as:
\begin{equation}
    \begin{aligned}
    \bx^{t+1}, \bv^{t+1}, \bF^{t+1}, \bC^{t+1} = \mathcal{S}(\bx^{t}, \bv^{t}, \bF^{t}, \bC^{t}, \bm{\theta}, \Delta t, N)  \\
    \end{aligned}
\end{equation}
where the timestamp $t+1$ is ahead of timestamp $t$ by $N \Delta t$. 
After simulation, we render the Gaussians at each frame:
\begin{equation}
    \hat{I}^{t} = \mathcal{F}_{\mathrm{render}} (\bx^{t}, \bm{\alpha}, \bm{R}^{t}, \Sigma, \bm{c}),
\end{equation}
where $\mathcal{F}_{\mathrm{render}}$ denotes the differentiable rendering function, and $\bm{R}^{t}$ denotes the rotation matrices of all particles obtained from the simulation step.  

Using the generated video as reference, we optimize the spatially-varying Young's modulus $\bm{E}$ and an initial velocity $\bv^0$ by a per-frame loss function:
\begin{equation}
\label{eq:rendering_loss}
L^t = \lambda L_{\mathrm{1}} (\hat{I}^t, I^t) + (1 - \lambda) L_{\mathrm{D-SSIM}} ( \hat{I}^t, I^t),
\end{equation}
where we set $\lambda=0.1$ in our experiments. Additionally, we adopt a total variation regularization for all spatial planes of both material field and velocity to encourage spatial smoothness. Using $\bu$ to denote one of the 2D spatial planes, $\bu$ we write the total variation regularization term as: 
\begin{equation}
    \label{eq:tv_regularization}
    L_{\text{tv}} = \sum_{i,j} \|\bu_{i+1, j} - \bu_{i,j}\|_2^2 + \|\bu_{i, j+1} - \bu_{i,j}\|_2^2,
\end{equation}
where $\bu_{i,j}$ is a feature vector on the 2D plane. 

Rather than optimizing the material parameters and initial velocity jointly, we split the optimization into two stages for better stability and faster convergence. 
In particular, in the first stage, we randomly initialize the Young's modulus for each Gaussian particle and freeze it. 
We optimize the initial velocity of each particle using only the first three frames of the reference video.  
In the second stage, we freeze the initial velocity and optimize the spatially varying Young's modulus. 
During the second stage, the gradient signal only flows to the previous frame to prevent gradient explosion/vanishing.



\subsection{Accelerate simulation with subsampling}

High-fidelity rendering with 3D Gaussian Splatting typically requires millions of particles to represent a scene. Running simulations on all the particles poses a significant computational burden. To improve efficiency, we introduce a subsampling procedure for simulation, as illustrated in Fig.~\ref{fig:subsample}.

Specifically, we apply K-Means clustering to create a set of driving particles $\{\mathcal{Q}_q\}_{q=1}^Q$ at $t=0$, where each driving particle is represented by $\mathcal{Q}^0_q = \{\bx^0_q, \bv^0_q, \bF^0_q, \bC^0_q, E_q, m_q, \nu_q, V_q\}$. 
The initial position of a driving particle $\bx_q^0$ is computed as the mean of the position $\bx_p$ of all cluster members. 
The number of the driving particles is much smaller than the number of 3D Gaussian particles, $Q \ll P$. 
We run simulations only on the driving particles. 
During rendering, we compute the position and rotation for each 3D Gaussian particle $\mathcal{G}_p$ by interpolating the driving particles. 
In particular, for each 3D Gaussian particle, we find its eight nearest driving particles at $t=0$, and we fit a rigid body transformation $\bm{T}$ between these eight driving particles at $t=0$ and at the current timestamp. This rigid body transformation $\bm{T}$ is applied to the initial position and rotation of the particle $\mathcal{G}_p$ to obtain its current position and rotation.

\input{fig_txt/fig_subsample}

% \subsection{Velocity and material fields} 

% Even with subsampling, the degree of freedom in the spatially-varying material is still high. In a typical scene, we have over ten thousand of driving particles, making the material estimation a highly ill-posed problem, where infinitely many solutions can lead to the same observation.

% To address this problem, we induce a spatial smoothness prior by representing the initial velocity and Young's modulus as implicit neural fields, $E_q=f_\text{material}(\bx_q)$ and $\bv^0_q=f_\text{velocity}(\bx_q)$, rather than directly optimizing discrete values for all driving particles. 
% In particular, we parameterize each field as tri-planes~\cite{peng2020convolutional,chan2022efficient} followed by a three-layer MLP. 

